A unified immersed finite element error analysis for one-dimensional interface problems

It has been noted that the traditional scaling argument cannot be directly applied to the error analysis of immersed finite elements (IFE) because, in general, the spaces on the reference element associated with the IFE spaces on different interface elements via the standard affine mapping are not the same. By analyzing a mapping from the involved Sobolev space to the IFE space, this article is able to extend the scaling argument framework to the error estimation for the approximation capability of a class of IFE spaces in one spatial dimension. As demonstrations of the versatility of this unified error analysis framework, the manuscript applies the proposed scaling argument to obtain optimal IFE error estimates for a typical first-order linear hyperbolic interface problem, a second-order elliptic interface problem, and the fourth-order Euler-Bernoulli beam interface problem, respectively.

==> Numerical_examples.tex <==
\section{Numerical examples}
 In this section, we present two computational examples to showcase the features of the IFE spaces for the kinematic wave equation. In addition to our examples, we refer the reader to \cite{adjeridHigherDegreeImmersed2018, moonImmersedDiscontinuousGalerkin2016} where a convergence rate of $O(h^{m+1})$ was observed numerically as predicted by our theory for the 1-D acoustic interface problem. For numerical examples on the approximation capabilities of the FE/IFE space described in \autoref{subsec:continuous_FE} and the convergence of the IFE method therein, we refer the reader to \cite{adjeridPthDegreeImmersed2009}. For numerical experiments for the Euler-Bernoulli beam interface problem, we refer the reader to \cite{linImmersedFiniteElement2011}.


\subsection{Kinematic wave equation with one interface}
Let us consider the following Transport equation with a discontinuous speed:
$$\begin{cases}
u_t(x,t)+c(x) u_x(x,t)=0,& t>0,\ x\in(0,\alpha)\cup(\alpha,4), \\
u(0,t)=0,&  t\ge 0,\\
u(x,0)=u_0(x),& x\in[0,4],
\end{cases}
\qquad c(x)=\begin{cases}
c_-,& x\le \alpha,\\
c_+,& x> \alpha,
\end{cases}\qquad c_{\pm}>0.
$$
For our first experiment, we choose $\alpha=\frac{\pi}{3}$, $(c_-,c_+)=(1,2)$ and $u_0(x)=f(3x-\frac{1}{2})$, where $f(x)=x(1-x^2)^5\mathbbm{1}_{[-1,1]}$. The exact solution to this problem is: 

$$u(x,t)=\begin{cases}
u_0(x-c_- t),& x\le \alpha, \\ 
\ds u_0\left(\frac{c_-}{c_+}\left(x-c_+ t\right)+\alpha\left(1-\frac{c_-}{c_+}\right)\right),& x> \alpha.
\end{cases}$$
We use our proposed IDG method for space discretization with  degree $m=1,2,3$ and adaptive RK45 for time integration on the time interval $[0,1]$. In \autoref{sufig:transport_L2_error}, we see that the $L^2$ error decays at an optimal rate of $O(h^{m+1})$. We also observe in \autoref{sufig:transport_spectral} that the largest stable choice of the time-step (i.e. the inverse of the spectral radius of the global IDG matrix) decays at a rate of $O(h)$.
\begin{figure}[ht]
\centering
    \begin{subfigure}{.3\textwidth}\centering
    \includegraphics[height=4cm]{figures/ex1 exact_soln.pdf}
    \caption{A plot of $u(x,0)$ (solid, red) and $u(x,1)$ (blue, dashed).}
    \end{subfigure}\qquad
     \begin{subfigure}{.3\textwidth}\centering
    \includegraphics[height=4cm]{figures/ex1 error_rate.pdf}
   
    \caption{$\norm{u-u_h}_{0,[0,4]}$ at $t=1$.}
     \label{sufig:transport_L2_error}
    \end{subfigure}\qquad
     \begin{subfigure}{.3\textwidth}\centering
    \includegraphics[height=4cm]{figures/ex1 spectral_radius.pdf}
    \caption{The largest $\Delta t$ that guarantees stability. }
     \label{sufig:transport_spectral}
    \end{subfigure}
    \label{fig:example_one}
    \caption{The exact solution (left), the $L^2$ error (middle) and the largest time-step $\Delta t$ (right)}
\end{figure}

We note that throughout this experiment, the relative position of $\alpha$ within the interface element denoted $\calpha\in(0,1)$ changes with $h$ but it does not affect the convergence rate. In the previous example, we have $0.02\le \calpha\le .75$ for $h=2^{-i}, i=3,\dots,9$. To show this more clearly, we fix $h=2^{-6}$ and use the previously mentioned value of $\alpha $ is in $I_{68}=[\frac{68}{2^6}, \frac{69}{2^6}]$. Instead of keeping $\alpha$ fixed, we vary $\alpha\in I_{68}$ (Hence, we vary $\calpha$ in $[0,1]$) and compute the $L^2$ error at $t=1$ the largest time-step $\Delta t$ for stability.  In  \autoref{fig:transport_varying_calpha}, we can observe that the relative position of the interface does not affect neither the $L^2$ error nor the largest stable time-step. 
\begin{figure}[ht]
\centering
     \begin{subfigure}{.3\textwidth}\centering
    \includegraphics[height=4cm]{figures/ex1 error_calpha.pdf}
    \caption{$\norm{u-u_h}_{0,[0,4]}$ at $t=1$.}
    \end{subfigure}\qquad
     \begin{subfigure}{.3\textwidth}\centering
    \includegraphics[height=4cm]{figures/ex1 spectral_calpha.pdf}
    \caption{The largest $\Delta t$ that guarantees stability. }
    \end{subfigure}
    \caption{The $L^2$ error (left) and the largest time-step $\Delta t$ (right) for different relative positions of the interface}
    \label{fig:transport_varying_calpha}
\end{figure}


\subsection{Kinematic equation with two interfaces}
Consider the following transport equation with two interfaces $\alpha_1<\alpha_2$ and periodic boundary conditions

$$\begin{cases}
u_t(x,t)+c(x) u_x(x,t)=0,& t>0,\ x\in(0,\alpha)\cup(\alpha,4), \\
u(0,t)=u(4,t),&  t\ge 0,\\
u(x,0)=u_0(x),& x\in[0,4],
\end{cases}
\qquad c(x)=\begin{cases}
c_-,& x\le \alpha_1,\\
c_+,& \alpha_1< x\le  \alpha_2,\\ 
c_-,& x>\alpha_2,\\ 
\end{cases},\qquad c_{\pm}>0.
$$
For the sake of simplicity, we will use the same $c_{\pm},u_0$ and we set $(\alpha_1,\alpha_2)=\left(\frac{\pi}{3},\frac{2\pi}{3}\right)$. Since $u(4,t)=u(0,t)$, the energy of the exact solution $\mathtt{E}(t)=\norm{\sqrt{S(\cdot)}\u(\cdot,t)}_{0,[0,4]}$ is constant and $u$ is periodic in time with period $\gamma=4-\frac{\pi}{6}\approx3.48$. To analyse the dissipation of our numerical scheme, we fix $h=2^{-6}$ and  plot the relative energy $\tilde{\mathtt{E}}_h(t)=\frac{\mathtt{E}_h(t)}{\mathtt{E}_h(0)}$ for $0\le t\le 10\gamma$, where $\mathtt{E}_h(t)=\norm{\sqrt{S(\cdot)}\u_h(\cdot,t)}_{0,[0,4]}$  in figure \autoref{fig:two_interfaces_dissipation}. We observe that our IDG method is dissipative when piecewise linear linear polynomials are used and highly conservative when higher order polynomials are used. For instance, for $m=2$, we have $1-\tilde{\mathtt{E}}_h(10\gamma)\le 2\cdot10^{-4}$, and for $m=3$, we have $1-\tilde{\mathtt{E}}_h(10\gamma)\le  10^{-8}$.

\begin{figure}[ht]
    \centering
    \includegraphics{figures/ex2 two_interfaces_dissipation.pdf}
    \caption{The relative dissipation $\tilde{\mathtt{E}}_h(t)$ for $0\le t\le 10\gamma$ and $m=1,2,3$.}
    \label{fig:two_interfaces_dissipation}
\end{figure}
